A Fast and Compact Invertible Sketch for Network-Wide Heavy Flow Detection

Fast detection of heavy flows (e.g., heavy hitters and heavy changers) in massive network traffic is challenging due to the stringent requirements of fast packet processing and limited resource availability. Invertible sketches are summary data structures that can recover heavy flows with small memory footprints and bounded errors, yet existing invertible sketches incur high memory access overhead that leads to performance degradation. We present MV-Sketch, a fast and compact invertible sketch that supports heavy flow detection with small and static memory allocation. MV-Sketch tracks candidate heavy flows inside the sketch data structure via the idea of majority voting, such that it incurs small memory access overhead in both update and query operations, while achieving high detection accuracy. We present theoretical analysis on the memory usage, performance, and accuracy of MV-Sketch in both local and network-wide scenarios. We further show how MV-Sketch can be implemented and deployed on P4-based programmable switches subject to hardware deployment constraints. We conduct evaluation in both software and hardware environments. Trace-driven evaluation in software shows that MV-Sketch achieves higher accuracy than existing invertible sketches, with up to 3.38x throughput gain. We also show how to boost the performance of MV-Sketch with SIMD instructions. Furthermore, we evaluate MV-Sketch on a Barefoot Tofino switch and show how MV-Sketch achieves line-rate measurement with limited hardware resource overhead.

==> fig/pdfcrop <==
#!/usr/bin/env perl

##    PDFCrop  version 0.4b
##    -------  ------- ----
## 
##  Copyright 2011 -- Eric Doviak <eric@doviak.net>
##  Copyright 2011 -- Tomas Janousek <tomi@nomi.cz>
## 
##  Eric Doviak wrote most of this Perl script, but Tomas Janousek wrote 
##  the template for the PDFedit script. Eric Doviak's work is copyrighted 
##  under the terms of the GPL v3. Janousek's work is copyrighted under 
##  the terms of the BSD license. The BSD licensed portions are denoted 
##  in the text of this script and the PDFedit script that this script
##  generates.


##  Syntax:   pdfcrop input.pdf [papersize] [output.pdf]
##  
##  Function: 
##    calculates the page metrics and scale factor of a PDF file, 
##    then crops and scales the PDF, so that it neatly fits on a 
##    standard size sheet of paper
##  
##  Options:
##    -h  --help  help      print usage and exit
##  
##    letter  Letter        if you want letter size paper
##    a4      A4            if you want A4 size paper 
##    legal   Legal         if you want legal size paper 
##  
##  Details:
##    pdfcrop attempts to determine your desired paper size by
##    reading /etc/papersize. If that file cannot be read, it 
##    assumes that you want letter size pages.
##  
##    If an output file name is not given, then pdfcrop assumes
##    that the input file should be cropped and scaled.
##  
##  Examples:
##    pdfcrop input.pdf
##    pdfcrop input.pdf A4 output.pdf

use strict ; 
use warnings ; 
no warnings qw( uninitialized ) ; 
use File::Copy ; 

## read arguments
my ( $infile , $pagesize , $otfile ) = read_arguments( @ARGV ) ; 

## create a randomly named directory in /tmp/
my $random = sprintf( "%04d" , int( 1000*rand() ) )  ; 
my $tmpdir = "/tmp/pdfcrop_$random/" ; 
mkdir( $tmpdir ) ; 

## if a different output file is desired, then create it
## all scripts will then operate on that output file, 
## so reset the input file name
if ( $infile ne $otfile ) {
    copy( $infile , $otfile ) ; 
    $infile = $otfile ; 
}

## names of script files
my $gsfile = $tmpdir . $infile . ".gs.out" ; 
my $qsfile = $tmpdir . $infile . ".fix.qs" ; 

## run ghostscript
open( BASH , "|/bin/bash") || die "could not open BASH" ; 
print BASH "gs -dSAFER -dNOPAUSE -dBATCH -q -r72 -sDEVICE=bbox -f $infile 2> $gsfile" ; 
close BASH ; 

## print the prologue
open( OVERWRITE , ">$qsfile" ) || die "could not overwrite $qsfile" ; 
print OVERWRITE make_prologue() ; 

## initialize page numbers
my $pagenumber = 1 ; 

## read the ghostscript file and create the script for "pdfedit"
open( GSFILE , $gsfile ) || die "could not read $gsfile" ; 
while (<GSFILE>) {

    chomp ; 
    my $line = $_ ; 

    if ( $line =~ /HiResBoundingBox: (\S+) (\S+) (\S+) (\S+)/ ) {

	## what are the borders? 
	my @borders = ($1 , $2 , $3 , $4) ; 

	## check for correctness
	check_borders( @borders ) ; 

	## print it all out
	my ( $hl , $vb , $hr , $vt ) = @borders ; 

	print OVERWRITE "runPDFcrop( doc , $pagenumber , \"$pagesize\" , $hl , $vb , $hr , $vt );\n" ;

	## increment the page number
	$pagenumber++ ; 
    }
}
close GSFILE ; 

## print the epilogue
print OVERWRITE make_epilogue() ; 
close OVERWRITE ; 

## crop and resize the pages
open( BASH , "|/bin/bash") || die "could not open BASH" ; 
print BASH "pdfedit -console -run $qsfile $infile 2> /dev/null" ; 
close BASH ; 

## get rid of junk
unlink( $gsfile , $qsfile ) ; 
rmdir( $tmpdir ) ; 


##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  
  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  
##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  ##  

## SUBROUTINES
## ===========

## read arguments

sub read_arguments {

    my @args = @_ ; 

    ## do you need help?
    if ( ! @args) {
	print_usage() ; 
    }

    foreach my $arg (@args) {
	if ( $arg =~ /^-h$|^--help$|^help$/ ) {
	    print_usage() ; 
	}
    }

    ## which arguments are PDF files? which are not
    my @pdffiles ; 
    my $pagesize ;

    foreach my $arg (@args) {
	if ( $arg =~ /pdf$/i ) {
	    push( @pdffiles , $arg ) ; 

	} elsif ( $arg =~ /^letter$|^legal$|^a4$/i ) {
	    $pagesize = lc( $arg ) ; 
	}
    }

    ## first PDF is assumed to be the input file
    my $infile = $pdffiles[0] ; 
    my $otfile ; 
    if ( ! $pdffiles[1] ) { 
	$otfile = $infile ;
	$otfile =~ s/pdf$/pdfcrop.pdf/i ; 
    } else {
	$otfile = $pdffiles[1] ;
    }

    ## if $infile is not a file, then there's an error
    if ( ! -f $infile ) {
	print "\n\tError! $infile not found.\n\n";
	print_usage() ; 
    }
    
    ## what is desired papersize? -- attempt to read "/etc/papersize"
    my $etc_papersize ; 
    if ( -f "/etc/papersize" ) {
	open( PAPERSIZE , "/etc/papersize" ) ; 
	chomp( $etc_papersize = <PAPERSIZE> ) ; 
	$etc_papersize = lc( $etc_papersize ) ; 
	close PAPERSIZE ; 
    } 

    ## if $pagesize not found, then check /etc/papersize
    ## if still not found, then assume "letter"    
    ## note: "papersize" vs. "pagesize" ... <roll eyes>
    if ( ! $pagesize ) {
	$pagesize = ( $etc_papersize !~ /^letter$|^legal$|^a4$/ ) ? "letter" : $etc_papersize ; 
    }
    
    my @otarray = ( $infile , $pagesize , $otfile ) ; 
    return @otarray ; 
}



## need a function that evaluates correctness of borders
sub check_borders {
    
    my @borders = @_[0..3] ; 
    my ( $hl , $vb , $hr , $vt ) = @borders ; 
    
    foreach my $border (@borders) {
	if ( ! is_float( $border )) {
	    die "Could not determine the Bounding Box borders."
	}
    }
    
    ## die if page has zero width or height
    if ( $hl == $hr || $vb == $vt ) { 
	
	print "\n" ; 
	if ( $hl == $hr ) { 
	    print "\tError! Bounding Box borders imply page width of zero.\n";
	}
	if ( $vb == $vt ) { 
	    print "\tError! Bounding Box borders imply page height of zero.\n";
	}
	print "\n" ; 
	die ; 
    }
}



## these two are modified versions from:
## http://stackoverflow.com/questions/12647/how-do-i-tell-if-a-variable-has-a-numeric-value-in-perl

sub is_integer {
    my $inval = $_[0] ; 
    defined $inval && $inval =~ /^[+-]?\d+$/;
}

sub is_float {
    my $inval = $_[0] ; 
    defined $inval && $inval =~ /^[+-]?\d+(\.\d+)?$/;
}



## we need prologue and epilogue for PDFedit script

sub make_prologue {
    
    my $text = <<END;

/* Beginning of BSD licensed code from Tomas Janousek. */
function setProp4( dict, p, a, b, c, d ) {
    if ( !dict.exist( p ) ) {
	var n = createArray();
	n.add( createReal( 0 ) );
	n.add( createReal( 0 ) );
	n.add( createReal( 0 ) );
	n.add( createReal( 0 ) );
	dict.add( p, n );
    }
    
    x = dict.property( p );
    x.property( 0 ).set( a );
    x.property( 1 ).set( b );
    x.property( 2 ).set( c );
    x.property( 3 ).set( d );
}
/* End of BSD licensed code from Tomas Janousek. */

function setScale( doc , pagenum , sx , sy ) {
    var pg = doc.getPage( pagenum ) ; 
    pg.setTransformMatrix([sx,0,0,sy,0,0]);
}


function runPDFcrop( doc, pagenum , papersize , hl , vb , hr , vt ) {

    dict = doc.getPage( pagenum ).getDictionary();
    
    /* get the MediaBox borders:  mbhl  mbvb  mbhr  mbvt */ 
    media = dict.property( "MediaBox" );
    mbhl = media.property( 0 ).value();
    mbvb = media.property( 1 ).value();
    mbhr = media.property( 2 ).value();
    mbvt = media.property( 3 ).value();

    /* determine orientation -- portrait or landscape */
    /* if horizontal longer then landscape, else portrait */
    if ( mbhr - mbhl > mbvt - mbvb ) { 
	if ( papersize == "letter" ) { 
	    pgwidth  =  792 ; 
	    pgheight =  612 ; 
	}
	if ( papersize == "legal" ) { 
	    pgwidth  = 1008 ; 
	    pgheight =  612 ;
	}
	if ( papersize == "a4" ) {
	    pgwidth  =  29.7 * 28.3464567 ;
	    pgheight =  21.0 * 28.3464567 ; 
	}
    } else {
	if ( papersize == "letter" ) {
	    pgwidth  =  612 ; 
	    pgheight =  792 ; 
	}
	if ( papersize == "legal" ) { 
	    pgwidth  =  612 ; 
	    pgheight = 1008 ;
	}
	if ( papersize == "a4" ) {
	    pgwidth  = 21.0 * 28.3464567 ; 
	    pgheight = 29.7 * 28.3464567 ;
	}
    }
    

    /*  now work with the borders of the bounding box    */

    /* we want 5 percent margins on each side */
    margins = 1.10 ; 
    
    /* get scale factor */
    horiz = pgwidth  / (margins*(hr-hl)) ;
    vert  = pgheight / (margins*(vt-vb)) ;
    
    if ( horiz < vert ) { 
	scale = horiz ; 
    } else {
	scale = vert  ;
    }
    
    /* find midpoints on the page */
    midh = ((hr - hl) / 2 ) + hl ;
    midv = ((vt - vb) / 2 ) + vb ;

    
    /* here are the new page metrics -- everything centered */
    nhl = ( midh * scale ) - ( pgwidth  / 2 ) ;
    nhr = nhl + pgwidth   ; 
    /* nvb = ( midv * scale ) - ( pgheight / 2 ) ;  */
    /* nvt = nvb + pgheight ;                       */

    /* alternative is to top-align the pages */
    halfmargin = 1 + (( margins - 1 )/2) ; 
    nvt = vt * scale * halfmargin ; 
    nvb = nvt - pgheight  ; 

    /* set CropBox, MediaBox and TrimBox. */
    setProp4( dict, "CropBox",  nhl, nvb, nhr, nvt ) ;
    setProp4( dict, "MediaBox", nhl, nvb, nhr, nvt ) ;
    setProp4( dict, "TrimBox",  nhl, nvb, nhr, nvt ) ;
   
    /* rescale the page */
    setScale( doc , pagenum , scale , scale );
}

doc = loadPdf( takeParameter(), false );
END

    return $text ; 
}

sub make_epilogue {

    my $text = <<END;
doc.save( false );
exit( 0 );
END

    return $text ; 
}

## print usage of this script

sub print_usage {

    my $program = "pdfcrop" ;

my $usage = <<"END_OF_USAGE";
Syntax:   \L$program\E input.pdf [papersize] [output.pdf]

Function: 
  calculates the page metrics and scale factor of a PDF file, 
  then crops and scales the PDF, so that it neatly fits on a 
  standard size sheet of paper

Options:
  -h  --help  help      print usage and exit

  letter  Letter        if you want letter size paper
  a4      A4            if you want A4 size paper 
  legal   Legal         if you want legal size paper 

Details:
  $program attempts to determine your desired paper size by
  reading /etc/papersize. If that file cannot be read, it 
  assumes that you want letter size pages.

  If an output file name is not given, then $program assumes
  that the input file should be cropped and scaled.

Examples:
  \L$program\E input.pdf
  \L$program\E input.pdf A4 output.pdf
END_OF_USAGE


    ## now print it out and quit 
    print "\n";
    print $usage ;
    die "\n"; 
}

